Probabilistic Modeling of LCF Failure Times Using an Epidemiological Crack Percolation Model

The analysis of standardized low cycle fatigue (LCF) experiments shows that the failure times widely scatter. Furthermore, mechanical components often fail before the deterministic failure time is reached. A possibility to overcome these problems is to consider probabilistic failure times. Our approach for probabilistic life prediction is based on the microstructure of the metal. Since we focus on nickel-base alloys we consider a coarse grained microstructure, with random oriented FCC grains. This leads to random distributed Schmid factors and different anisotropic stress in each grain. To gain crack initiation times, we use Coffin-Manson- Basquin and Ramberg-Osgood equation on stresses corrected with probabilistic Schmid factors. Using these single grain crack initiation times, we have developed an epidemiological crack growth model over multiple grains. In this mesoscopic crack percolation model, cracked grains induce a stress increase in neighboring grains. This stress increase is realized using a machine learning model trained on data generated from finite element simulations. The resulting crack clusters are evaluated with a failure criterion based on a multimodal stress intensity factor. From the generated failure times, we calculate surface dependent hazard rates using a Monte Carlo framework. We compare the obtained failure time distributions to data from LCF experiments and find good coincidence of predicted and measured scatter bands.

==> section_7_ECCOMASGUIDLINES.tex <==
The Full Paper must be written in English within a printing box of 16cm x 21cm, centered in the page. The Full Paper including figures, tables and references must have a minimum length of 6 pages and must not exceed 12 pages. Maximum file size is 4 MB.

\section{TITLE, AUTHORS, AFFILIATION, KEY WORDS}

The first page must contain the Title, Author(s), Affiliation(s),
Key words and the Summary. The Introduction must begin immediately
below, following the format of this template.

\subsection{Title}

The title should be written centered, in 14pt, boldface Roman, all
capital letters. It should be single spaced if the title is more
than one line long.

\subsection{Author}

The author's name should include first name, middle initial and
surname. It should be written centered, in 12pt boldface Roman,
12pt below the title.

\subsection{Affiliation}

Author's affiliation should be written centered, in 11pt Roman,
12pt below the list of authors. A 12pt space should separate two
different affiliations.

\subsection{Key words}

Please, write no more than six key words. They should be written
left aligned, in 12pt Roman, and the line must begin with the
words {\bf Key words}: boldfaced. A 12pt space should separate the
key words from the affiliations.

\subsection {Summary (optional)}

Use 12pt Italic Roman for the summary. The word {\bf Summary} must
be set in boldface, not italicized, at the beginning of the first
line. The text should be justified and separated 12pt from the key
words, as shown in the first page of these instructions.

\section{HEADINGS}

\subsection{Main headings}

The main headings should be written left aligned, in 12pt,
boldface and all capital Roman letters. There should be a 12pt
space before and 6pt after the main headings.

\subsection {Secondary headings}

Secondary headings should be written left aligned, 12 pt, boldface
Roman, with an initial capital for first word only. There should
be a 12pt space before and 6pt after the secondary headings.

\section{EDITORIAL HEADING}

The first page has to include the Editorial Heading, as shown in
the first page of these instructions. Successive pages will
include the name of the authors.

\section{TEXT}

The normal text should be written single-spaced, justified, using
12pt (Times New) Roman in one column. The first line of each
paragraph must be indented 0.5cm. There is not inter-paragraph
spacing.

\section{PAGE NUMBERS}

In order to organize the Full Paper, it is better to number
the pages. Page numbers are not included in the printing box.

\section{FIGURES}

All figures should be numbered consecutively and captioned. The
caption title should be written centered, in 10pt Roman, with
upper and lower case letters.

\begin{figure}[t]
\centering
\includegraphics[width=11cm]{firstpage}
\caption{Page layout}
\end{figure}

A 6pt space should separate the figure from the caption, and a
12pt space should separate the upper part of the figure and the
bottom of the caption from the surrounding text.

Figures may be included in the text or added at the bottom of the paper.

\section{EQUATIONS}

A displayed equation is numbered, using Arabic numbers in
parentheses. It should be centered, leaving a 6pt space above and
below to separate it from the surrounding text.

The following example is a single line equation:
\vskip-.6cm
\begin{eqnarray}
Ax = b
\end{eqnarray}

The next example is a multi-line equation:
\vskip-.6cm
\begin{eqnarray}
Ax = b \\
Ax = b \nonumber
\end{eqnarray}

\section{TABLES}

All tables should be numbered consecutively and captioned, the
caption should be 10pt Roman, upper and lower case letters.

\begin{table}[h!]
\caption{Example of the construction of one table}
\begin{center}
\begin{tabular}{*{3}{c}}
\hline
C11 & C12 & C13 \\
\hline
C21 & C22 & C23 \\
\hline
C31 & C32 & C33 \\
\hline
C41 & C42 & C43 \\
\hline
C51 & C52 & C53 \\
\hline
\end{tabular}
\end{center}
\end{table}

A 6pt space should separate the table from the caption, and a 12pt
space should separate the table from the surrounding text.

\section{FORMAT OF REFERENCES}

References should be quoted in the text by superscript
numbers \cite{Zienkiewicz,Idelsohn} and grouped together at the end of the Full Paper in numerical order as shown in these instructions.

\section{CONCLUSIONS}

\begin{itemize}
\item[-] Full Papers in format \cite{GottschSchmitz_2012} for publication should be submitted electronically via the web page of the Conference, before \textbf{June 1st 2022}. The file must be converted to  Portable Document Format (PDF) before submission. The maximum size of the file is 4 Mb.



\end{itemize}
\todo{Bitte Literatur umstellen auf BibTeX -- zB .bib-file von Lucas Thesis verwenden}



\begin{thebibliography}{99}

\bibitem{Zienkiewicz}  Zienkiewicz, O.C. and  Taylor, R.L. \textit{The finite element method}. McGraw Hill,
Vol. I., (1989), Vol. II., (1991).
\bibitem{Idelsohn} Idelsohn, S.R. and O\~{n}ate, E. Finite element and finite volumes. Two good friends.
\textit{Int. J. Num. Meth. Engng.} (1994) \textbf{37}:3323--3341.
\bibitem{Moch} Moch, Nadine, From Microscopic Models of Damage Accumulation to the Probability of Failure of Gas Turbines, (2019) doi:10.25926/mfaj-nq46.
\bibitem{Engel}  B. Engel, L. M\"ade, P. Lion, N. Moch, H. Gottschalk and T. Beck, \textit{Probabilistic Modeling of Slip System-Based Shear Stresses and Fatigue Behavior of Coarse-Grained Ni-Base Superalloy Considering Local Grain Anisotropy and Grain Orientation}, Metals - Open Access Metallurgy Journal Vol. \textbf{9} (8), 2019. 
\bibitem{Made} L. M\"ade, S. Schmitz, H. Gottschalk and T. Beck, Combined \textit{ Notch and Size Effect Modeling in a Local Probabilistic Approach for LCF}, Computational Materials Science, 2017
\bibitem{Gott} H. Gottschalk, S. Schmitz, T. Seibel, G. Rollmann, R. Krause and T. Beck, \textit{Probabilistic Schmid factors and scatter of low cycle fatigue (LCF) life}, Materialwissenschaft und Werkstofftechnik. 9999,  2015
\end{thebibliography}


==> tikz_overview.tex <==
\begin{tikzpicture}[
node distance = 12mm and 12mm, 
   box/.style = {draw, rounded corners, 
                 minimum width=22mm, minimum height=5mm, align=center},
            > = {Straight Barb[angle=60:2pt 3]},
   bend angle = 15,
         auto = right,
                        ]
\node (n1)  [box] {FEM-Simulations};
\node (n2)  [box, below right=of n1]    {Voronoi Tesselation};
\node (n3)  [box, right=of n2]    {Probebalistic Schimd Factors};
\node (n4)  [box, above right=of n2] {ML-Model};
\node (n5) 	[box, right=of n3] {Corrected Stress};
\node (n6) 	[box, right=of n5] {K Factor};
\node (n7) 	[box] at (22,-1) {Fitting};
\coordinate (Qf) at ([xshift=-0.5cm]n5.west);
%
\draw (n4) -- (Qf) -- (n5);
\draw[->]        (n2) to  (n3);
\draw[->]        (n3) to   (n5);
\draw[->] 	     (n1) to (n4);
\draw[->]        (n5) to  (n6);
\draw[->]		(19.5,-1) -- (20.9,-1) node[midway] {MC};
\draw[blue,thick,dotted] ($(n2.north west)+(-0.3,2.3)$)  rectangle ($(n6.south east)+(0.3,-0.6)$);
\end{tikzpicture}
